A Practical Examination of AI-Generated Text Detectors for Large Language Models

The proliferation of large language models has raised growing concerns about their misuse, particularly in cases where AI-generated text is falsely attributed to human authors. Machine-generated content detectors claim to effectively identify such text under various conditions and from any language model. This paper critically evaluates these claims by assessing several popular detectors (RADAR, Wild, T5Sentinel, Fast-DetectGPT, PHD, LogRank, Binoculars) on a range of domains, datasets, and models that these detectors have not previously encountered. We employ various prompting strategies to simulate practical adversarial attacks, demonstrating that even moderate efforts can significantly evade detection. We emphasize the importance of the true positive rate at a specific false positive rate (TPR@FPR) metric and demonstrate that these detectors perform poorly in certain settings, with TPR@.01 as low as 0%. Our findings suggest that both trained and zero-shot detectors struggle to maintain high sensitivity while achieving a reasonable true positive rate.

==> sections/05_attack.tex <==
\section{Results and Analysis}

\subsection{Plain Prompting}
We evaluate the AUROC and TPR at FPR rates of .01 and .1 for machine generated texts from direct prompting using identical prompts as human written texts. A simple prompt was employed to ensure the generated text was in the correct format.

% \begin{figure}[t]
% \centering
% \begin{minipage}[T]{0.55\textwidth}
% \resizebox{\linewidth}{!}{
% \centering
% \begin{tabular}{lllll}
% \toprule
% \multicolumn{2}{c}{} & \multicolumn{3}{c}{\textbf{Metrics}} \\ 
% \textbf{Model} & \textbf{Detector} & \textbf{TPR@.01} & \textbf{TPR@.10} & \textbf{AUROC} \\ \midrule
% \multirow{4}{*}{GPT-4} & RADAR & 0.05 & 0.46 & 0.8527 \\  
%  & Wild & 0.00 & 0.39 &  0.8561 \\  
%  & Fast-DetectGPT & 0.00 & 0.92 & 0.9323 \\  
%  & GPTID & 0.00 & 0.03 &  0.4252 \\ \midrule
% \multirow{4}{*}{Mixtral1} & RADAR & 0.34 & 0.73 & 0.9234 \\ 
%  & Wild & 0.00 & 0.51 & 0.8641 \\
%  & Fast-DetectGPT & 0.00 & 0.75 &  0.9003 \\ 
%  & GPTID & 0.00 & 0.02 & 0.1426 \\ \bottomrule
% \end{tabular}
% }
% \captionof{table}{TPR@.01FPR, TPR@.1FPR, and AUROC scores for GPT-4 and Mistral. Due to budget constraints, these models are not included in the aggregate table. However, it is essential to present the metrics for the current highest-performing LLMs. The AUROC scores for these two models are slightly lower than the other models, but the difference is not significant. Furthermore, the TPR@.01FPR and TPR@.10FPR scores are consistent with the other models.}
% \label{tab:gpt4mixtral}
% \end{minipage}
% \hfill
% \begin{minipage}[T]{0.43\textwidth}
% \begin{figure}[H]
%     \centering
% \includegraphics[width=0.9\linewidth]{figures/AvgPearson.png}
%     \caption{Average Pearson correlation with AUROC across domains for each false positive rate threshold. FPRs close to 0 and close to 1 are much less correlated with the AUROC score. The AUROC is more representative of the 50\% FPR and masks over the 1\% FPR.}
%     \label{fig:corr}
% \end{figure}
% \end{minipage}
% % \vspace{-1.5em}
% \end{figure}

Table \ref{tab:performance} presents the results. Notably, there are significant differences between the scores of detectors across tasks. The most pronounced difference was a 78\% drop in the AUROC score of GPTID between the code and question-answering tasks. Even Fast-DetectGPT, the highest performing detector overall, exhibited a 23\% decrease in summarization performance compared to its multilingual performance. The translation scores are ignored due to significantly shorter response lengths, resulting in nearly random guessing performance. Table \ref{tab:gpt4mixtral} separately illustrates the results for Mixtral and GPT4, as budget constraints prevented running the results for all tasks.

Another notable finding is the low TPR@FPR given high AUROC. For instance, in the question-answering task, both RADAR and Fast-DetectGPT achieve similar AUROC scores of .9608 and .9471, respectively. However, they have a large gap between their TPR@.01 scores of 0.39 and 0.0, respectively. 

These results highlight two issues with using AUROC as a metric for detectors. First, its inability to discriminate between detectors, as there can be a significant performance gap despite similar AUROC scores. Second, its inability to predict practical performance, as high AUROC scores do not necessarily translate to real-world usability. For example, an FPR of 1\% or lower is required in this domain, but a TPR of 0\% at an FPR of 1\% renders the detector impractical. Figure \ref{fig:corr} shows the correlation between the TPR at different FPRs and the AUROC score. The AUROC score accurately represents the TPR@.3-.55 but falls off at the edges. The TPR@.01 does not have a meaningful correlation with AUROC when compared the middle of this curve. As previously described, the most important aspect of these detectors is their ability to detect while keeping a low FPR and the AUROC does not consistently portray that ability.






\subsection{Prompting with Adversarial Prompt}

Table \ref{tab:template_performance} shows the results of the detectors on the model output using adversarial prompting. Overall, there was not much difference between the normal prompts and the scenario-based adversarial prompts attempting to get the model to be more human-like. In many cases, the text was easier to detect as machine-generated. None of the tasks show any significant difference from any other the others. Additionally, none of the detectors behave consistently across detectors. This all indicates that a request that the model pretends to be human actually makes the output less human-like.

This has some important implications for adversarial prompting in practice. The most obvious method that is likely used in practice is simply asking the language model to be more human like. As shown by these results, it will not actually make it more human, at least not by the standards of detectors. These results raise two interesting questions for us: Can any rephrasing of the question provide less detectable output and what is a language models perception of "human text"? We propose to answer the first question with the results of our PAIR attack and leave the second question for future work.


% \subsection{PAIR Attack}

% % \begin{table*}[t]

% \begin{table}
% \setlength{\tabcolsep}{1.5pt}
% \centering
% \resizebox{0.6\linewidth}{!}{
% \begin{tabular}{lllcccc}
% \toprule
% \multirow{2}{*}{\textbf{Attacker}} & \multirow{2}{*}{\textbf{Target}} & \multirow{2}{*}{\textbf{Detector}} & \multicolumn{2}{c}{\textbf{QA}} & \multicolumn{2}{c}{\textbf{Target QA}}\\ 
% & &  & TPR@.01 $\uparrow$& AUROC $\uparrow$  & TPR@.01 $\uparrow$ & AUROC $\uparrow$\\
% \midrule
% \multirow{1}{*}{Mistral-7B} & \multirow{1}{*}{Vicuna-13B} &
% RADAR & 0.28& 0.9467  & 0.43& 0.9635 \\ 

% \multirow{1}{*}{Mistral-7B} & \multirow{1}{*}{Vicuna-13B} &
% Wild & 0.00& 0.9348  & 0.03& 0.9161 \\   

% \multirow{1}{*}{Mistral-7B} & \multirow{1}{*}{Vicuna-13B} &
% Fast-DetectGPT & 0.00& 0.9094  & 0.00& 0.9533 \\  

% \multirow{1}{*}{Vicuna-13B} & \multirow{1}{*}{Mistral-7B} &
% Wild & 0.01& 0.8784  & 0.03& 0.8984 \\  

% \multirow{1}{*}{Mistral-7B} & \multirow{1}{*}{Mistral-7B} &
% Wild & 0.01& 0.9024  & 0.03& 0.8984 \\  
% \bottomrule
% \end{tabular}
% }
% \vspace{-0.5em}
% \caption{AUROC and TPR@.01 scores for the generated text using the PAIR method. The attacker represents the prompting model, while the target is the model generating the final text. Target QA provides reference scores for the target model using the original text.}
% \label{table:PAIR}
% % \end{table*}
% \end{table}

% For the PAIR attack, we gathered metrics from the question-answering domain in 5 different settings. As shown in Table
% \ref{table:PAIR}, the results did not shift the distribution of the generator model outputs significantly. The TPR@.01 remained low in most cases, except for the RADAR detector, which is consistent with what we see in Table \ref{tab:performance}. For a more specific comparison, Table \ref{table:PAIR} also shows the detector performance on only the target models' outputs. While not a large experiment, this gives a strong indication that prompt engineering, at least from another language model, is not a very successful technique for making machine-generated text less detectable. This is a surprising result, however, because this same method has had good success in jailbreaking language models, as shown by \citet{chao2023jailbreaking}. This provides evidence that post processing on text will be a much more efficient method for evading text detectors.



% \subsection{Paraphrasing Attack}
% % \begin{table}[htbp]
% \begin{table}
% \small
% \centering
% \begin{tabular}{lll}
% \toprule
% \textbf{Model} & \textbf{TPR@.01} & \textbf{AUROC} \\ \midrule
% RADAR & 0.33  & 0.9692 \\ 
% Wild & 0.03  & 0.8984 \\ 
% Fast-DetectGPT & 0.00  & 0.9533 \\ 
% GPTID & 0.00 & 0.0911 \\ \bottomrule
% \end{tabular}
% \caption{TPR@.01FPR and AUROC scores for Mistral generation on each detector.
% % This table enables comparison with the results presented in the paraphrase table.
% }
% \label{tab:mistral_results}
% % \end{table}
% \end{table}
% We also gathered experimental results for the paraphrasing setting shown in Table \ref{table:paraphrase_results}. We considered four different settings under the question-answering tasks, where the original generator is a model that all of the detectors have seen before, and the paraphrasing model is a model that the detectors have not seen before. For comparison, we also included the scores from the Generation model. Table \ref{tab:mistral_results} includes the scores for the paraphrasing model on the question-answering task for each detector.

% These results do not show any strong indication that this simple paraphrasing method makes the text harder to detect. They do show that the detectability is at least different than either of the models on their own. This is intuitive because the generation model is answering the question in its own style and the paraphrasing model is adding its own style. The merging of these styles creates a new style that is not any more detectable as AI generated or human generated.


% \begin{table}[h]
% \setlength{\tabcolsep}{3.5pt}
% \centering
% \resizebox{0.85\linewidth}{!}{
% \begin{tabular}{cclcccc}
% \toprule
% \multirow{2}{*}{\textbf{Generator}} & \multirow{2}{*}{\textbf{Paraphraser}} & \multirow{2}{*}{\textbf{Detector}} & \multicolumn{2}{c}{\textbf{QA}} & \multicolumn{2}{c}{\textbf{Gen QA}}\\ 
% & & & TPR@.01 $\uparrow$ & AUROC $\uparrow$ & TPR@.01 $\uparrow$ & AUROC $\uparrow$ \\
% \midrule
% \multirow{4}{*}{Llama2-13B} & \multirow{4}{*}{Mistral-7B} &
% RADAR & 0.11 & 0.9199 & 0.12 & 0.9198\\  
%  & & Wild & 0.14 & 0.9439 & 0.14 & 0.8984\\ 
%  & & Fast-DetectGPT & 0.00 & 0.9414 & 0.00 & 0.9533\\ 
%  & & GPTID & 0.00 & 0.0899 & 0.00 & 0.0914 \\  
%  \midrule
% \multirow{4}{*}{Vicuna-13B} & \multirow{4}{*}{Mistral-7B} &
% RADAR & 0.38 & 0.9647 & 0.43 & 0.9635\\  
%  & & Wild & 0.02 & 0.9045 & 0.03 & 0.9161\\ 
%  & & Fast-DetectGPT & 0.00 & 0.9424 & 0.00 & 0.9547\\ 
%  & & GPTID & 0.00 & 0.1134 & 0.00 & 0.1293\\  
%   \midrule
% \multirow{2}{*}{Llama2-13B} & \multirow{4}{*}{Mistral-7B} &
% RADAR & 0.11 & 0.9014 & 0.00 & 0.8321\\  
%  & & Wild & 0.09 & 0.9301 & 0.00 & 0.9001\\ 
%  \multirow{2}{*}{(Template)} & & Fast-DetectGPT & 0.00 & 0.9618 & 0.00 & 0.9650\\ 
%  & & GPTID & 0.00 & 0.1040 & 0.00 & 0.1620\\  
%   \midrule
% \multirow{2}{*}{Vicuna-13B} & \multirow{4}{*}{Mistral-7B} &
% RADAR & 0.33 & 0.9582 & 0.04 & 0.9864\\  
%  & & Wild & 0.03 & 0.8833 & 0.00 & 0.8500\\ 
%  \multirow{2}{*}{(Template)}& & Fast-DetectGPT & 0.00 & 0.9238 & 0.00 & 0.9650\\ 
%  & & GPTID & 0.00 & 0.1325 & 0.00 & 0.3974\\ 
% \bottomrule
% \end{tabular}
% }
% \caption{TPR@.01FPR and AUROC scores for the paraphrase attack. The generator is the model that initially generated the text, while the paraphraser is the model that paraphrased the text. Gen QA provides reference scores for the original text generated by the generator. Reference scores for the paraphrase model can be found in Table \ref{tab:mistral_results}.}
% \label{table:paraphrase_results}
% \end{table}






% \multirow{4}{*}{Llama2-13B} & 
% RADAR & 0.8321 & 0 & 0.8328 & 0.05 & 0.4595 & 0.04\\  
%  & Wild & 0.9001 & 0 & 0.6367 & 0.01 & 0.7312 & 0.06\\ 
%  & Fast-DetectGPT & 0.9650 & 0 & 0.9973 & 0.95 & 0.9935 & 0.95\\ 
%  & GPTID & 0.1620 & 0 & 0.9098 & 0.16 & 0.1647 & 0\\ 
%  \midrule
% \multirow{4}{*}{Vicuna-13B-v1.5} &
% RADAR & 0.9864 & 0.04 & 0.7081 & 0.02 & 0.6389 & 0.19\\  
%  & Wild & 0.8500 & 0 & 0.5778 & 0.02 & 0.5225 & 0.08\\ 
%  & Fast-DetectGPT & 0.9650 & 0 & 0.9963 & 0.94 & 0.9966 & 0.96\\ 
%  & GPTID & 0.3974 & 0 & 0.8208 & 0 & 0.3816 & 0\\ 
%   \midrule





==> sections/06_defense.tex <==
\section{Defense}








